Right On Q: Recovering Reasoning under Quantization via Self-Generated Trajectories

Quantization-aware training (QAT) aims to recover reasoning capabilities in low-bit large language models (LLMs). Existing recipes typically supervise the quantized student with the original full-precision model on fixed response sequences. However, the resulting low-bit quantized models still struggle on long-horizon reasoning tasks and often fail to terminate within a token budget that suffices for the full-precision model. We identify two challenges in closing this gap. First, fixed-response supervision leaves a mismatch between training prefixes and those encountered during student generation, and this trajectory divergence grows as responses lengthen. Second, on its own prefixes, the student underpredicts some next-token candidates and overpredicts others, and this distributional misalignment becomes more frequent at high-entropy prefixes. We present OnQ, a low-bit recovery pipeline that combines on-policy distillation and candidate-wise Dynamic KL. Starting from block-wise calibration, the quantized student generates responses and receives full-precision teacher supervision on its own prefixes. Dynamic KL weights forward and reverse KL by each candidate's teacher-student probability ratio to balance correction of under- and overprediction. Across Qwen3-1.7B, 4B, and 8B at 2- and 3-bit precision, OnQ achieves the highest nine-benchmark average, with the largest gains on long-horizon reasoning benchmarks. At 2 bits, it outperforms every baseline on every benchmark at every model size, improving the Qwen3-8B average by 10.26 points over the strongest baseline. It also produces shorter responses with fewer truncations and repetitive errors.

==> figures/paper_palette.tex <==
\definecolor{qatBlue}{HTML}{0072B2}
\definecolor{qatOrange}{HTML}{D55E00}
\definecolor{qatTeal}{HTML}{009E73}
\definecolor{qatPurple}{HTML}{CC79A7}
\definecolor{qatSky}{HTML}{56B4E9}
\definecolor{qatRef}{HTML}{222222}
\colorlet{qatAuto}{qatPurple}
\colorlet{qatCalib}{qatSky}
\colorlet{qatAuthor}{qatTeal}
\colorlet{qatKD}{qatOrange}
\colorlet{qatOPD}{qatBlue}
\definecolor{qatCorrect}{HTML}{6699CC}
\definecolor{qatWrong}{HTML}{EEAA88}
\definecolor{qatCap}{HTML}{994455}
\colorlet{qatLenA}{qatCorrect}
\definecolor{qatLenB}{HTML}{CCDDEE}
\colorlet{qatLenC}{qatWrong}
\colorlet{qatLenD}{qatCap}
\colorlet{tch}{qatRef}
\colorlet{stu}{qatBlue}
\colorlet{fklc}{qatOrange}
\colorlet{rklc}{qatTeal}
\colorlet{dklc}{qatBlue}
\definecolor{rrdStepA}{HTML}{00466E}
\definecolor{rrdStepB}{HTML}{0072B2}
\definecolor{rrdStepC}{HTML}{4C9CC9}
\definecolor{rrdStepD}{HTML}{8DC1DE}
\definecolor{rrdLogit}{HTML}{59A3CD}
\colorlet{rrdGrad}{qatOrange}

